SDRT: Enhance Vision-Language Models by Self-Distillation with Diverse Reasoning Traces

Reasoning is increasingly crucial for various tasks. While chain-of-thought prompting enables large language models to leverage reasoning effectively, harnessing the reasoning capabilities of Vision-Language Models (VLMs) remains challenging. To solve this problem, we propose a novel self-distillation framework that enhances the reasoning capabilities of the model. The proposed framework introduces several key innovations. We start by employing a prompt library tailored to visual reasoning tasks to generate diverse in-context questions and utilize a two-step reasoning procedure to derive reasoning-guided responses. These responses are then used for self-distillation, enabling the model to internalize the reasoning process. Additionally, we improve the model architecture with several innovative components, including an intervention adapter for efficient parameter updates, a cross-modal skip connection to facilitate information exchange between modalities, and an ensemble learning algorithm to integrate diverse reasoning from multiple in-context questions. Extensive experiments show that our method significantly improves the baseline performance across five VQA datasets.

==> backup/instructions.tex <==
\section{Submission of conference papers to ICLR 2024}

ICLR requires electronic submissions, processed by
\url{https://openreview.net/}. See ICLR's website for more instructions.

If your paper is ultimately accepted, the statement {\tt
  {\textbackslash}iclrfinalcopy} should be inserted to adjust the
format to the camera ready requirements.

The format for the submissions is a variant of the NeurIPS format.
Please read carefully the instructions below, and follow them
faithfully.

\subsection{Style}

Papers to be submitted to ICLR 2024 must be prepared according to the
instructions presented here.

%% Please note that we have introduced automatic line number generation
%% into the style file for \LaTeXe. This is to help reviewers
%% refer to specific lines of the paper when they make their comments. Please do
%% NOT refer to these line numbers in your paper as they will be removed from the
%% style file for the final version of accepted papers.

Authors are required to use the ICLR \LaTeX{} style files obtainable at the
ICLR website. Please make sure you use the current files and
not previous versions. Tweaking the style files may be grounds for rejection.

\subsection{Retrieval of style files}

The style files for ICLR and other conference information are available online at:
\begin{center}
   \url{http://www.iclr.cc/}
\end{center}
The file \verb+iclr2024_conference.pdf+ contains these
instructions and illustrates the
various formatting requirements your ICLR paper must satisfy.
Submissions must be made using \LaTeX{} and the style files
\verb+iclr2024_conference.sty+ and \verb+iclr2024_conference.bst+ (to be used with \LaTeX{}2e). The file
\verb+iclr2024_conference.tex+ may be used as a ``shell'' for writing your paper. All you
have to do is replace the author, title, abstract, and text of the paper with
your own.

The formatting instructions contained in these style files are summarized in
sections \ref{gen_inst}, \ref{headings}, and \ref{others} below.

\section{General formatting instructions}
\label{gen_inst}

The text must be confined within a rectangle 5.5~inches (33~picas) wide and
9~inches (54~picas) long. The left margin is 1.5~inch (9~picas).
Use 10~point type with a vertical spacing of 11~points. Times New Roman is the
preferred typeface throughout. Paragraphs are separated by 1/2~line space,
with no indentation.

Paper title is 17~point, in small caps and left-aligned.
All pages should start at 1~inch (6~picas) from the top of the page.

Authors' names are
set in boldface, and each name is placed above its corresponding
address. The lead author's name is to be listed first, and
the co-authors' names are set to follow. Authors sharing the
same address can be on the same line.

Please pay special attention to the instructions in section \ref{others}
regarding figures, tables, acknowledgments, and references.


There will be a strict upper limit of 9 pages for the main text of the initial submission, with unlimited additional pages for citations. 

\section{Headings: first level}
\label{headings}

First level headings are in small caps,
flush left and in point size 12. One line space before the first level
heading and 1/2~line space after the first level heading.

\subsection{Headings: second level}

Second level headings are in small caps,
flush left and in point size 10. One line space before the second level
heading and 1/2~line space after the second level heading.

\subsubsection{Headings: third level}

Third level headings are in small caps,
flush left and in point size 10. One line space before the third level
heading and 1/2~line space after the third level heading.

\section{Citations, figures, tables, references}
\label{others}

These instructions apply to everyone, regardless of the formatter being used.

\subsection{Citations within the text}

Citations within the text should be based on the \texttt{natbib} package
and include the authors' last names and year (with the ``et~al.'' construct
for more than two authors). When the authors or the publication are
included in the sentence, the citation should not be in parenthesis using \verb|\citet{}| (as
in ``See \citet{Hinton06} for more information.''). Otherwise, the citation
should be in parenthesis using \verb|\citep{}| (as in ``Deep learning shows promise to make progress
towards AI~\citep{Bengio+chapter2007}.'').

The corresponding references are to be listed in alphabetical order of
authors, in the \textsc{References} section. As to the format of the
references themselves, any style is acceptable as long as it is used
consistently.

\subsection{Footnotes}

Indicate footnotes with a number\footnote{Sample of the first footnote} in the
text. Place the footnotes at the bottom of the page on which they appear.
Precede the footnote with a horizontal rule of 2~inches
(12~picas).\footnote{Sample of the second footnote}

\subsection{Figures}

All artwork must be neat, clean, and legible. Lines should be dark
enough for purposes of reproduction; art work should not be
hand-drawn. The figure number and caption always appear after the
figure. Place one line space before the figure caption, and one line
space after the figure. The figure caption is lower case (except for
first word and proper nouns); figures are numbered consecutively.

Make sure the figure caption does not get separated from the figure.
Leave sufficient space to avoid splitting the figure and figure caption.

You may use color figures.
However, it is best for the
figure captions and the paper body to make sense if the paper is printed
either in black/white or in color.
\begin{figure}[h]
\begin{center}
%\framebox[4.0in]{$\;$}
\fbox{\rule[-.5cm]{0cm}{4cm} \rule[-.5cm]{4cm}{0cm}}
\end{center}
\caption{Sample figure caption.}
\end{figure}

\subsection{Tables}

All tables must be centered, neat, clean and legible. Do not use hand-drawn
tables. The table number and title always appear before the table. See
Table~\ref{sample-table}.

Place one line space before the table title, one line space after the table
title, and one line space after the table. The table title must be lower case
(except for first word and proper nouns); tables are numbered consecutively.




\begin{table}[t]
\caption{Sample table title}
\label{sample-table}
\begin{center}
\begin{tabular}{ll}
\multicolumn{1}{c}{\bf PART}  &\multicolumn{1}{c}{\bf DESCRIPTION}
\\ \hline \\
Dendrite         &Input terminal \\
Axon             &Output terminal \\
Soma             &Cell body (contains cell nucleus) \\
\end{tabular}
\end{center}
\end{table}


\section{Default Notation}

In an attempt to encourage standardized notation, we have included the
notation file from the textbook, \textit{Deep Learning}
\cite{goodfellow2016deep} available at
\url{https://github.com/goodfeli/dlbook_notation/}.  Use of this style
is not required and can be disabled by commenting out
\texttt{math\_commands.tex}.


\centerline{\bf Numbers and Arrays}
\bgroup
\def\arraystretch{1.5}
\begin{tabular}{p{1in}p{3.25in}}
$\displaystyle a$ & A scalar (integer or real)\\
$\displaystyle \va$ & A vector\\
$\displaystyle \mA$ & A matrix\\
$\displaystyle \tA$ & A tensor\\
$\displaystyle \mI_n$ & Identity matrix with $n$ rows and $n$ columns\\
$\displaystyle \mI$ & Identity matrix with dimensionality implied by context\\
$\displaystyle \ve^{(i)}$ & Standard basis vector $[0,\dots,0,1,0,\dots,0]$ with a 1 at position $i$\\
$\displaystyle \text{diag}(\va)$ & A square, diagonal matrix with diagonal entries given by $\va$\\
$\displaystyle \ra$ & A scalar random variable\\
$\displaystyle \rva$ & A vector-valued random variable\\
$\displaystyle \rmA$ & A matrix-valued random variable\\
\end{tabular}
\egroup
\vspace{0.25cm}

\centerline{\bf Sets and Graphs}
\bgroup
\def\arraystretch{1.5}

\begin{tabular}{p{1.25in}p{3.25in}}
$\displaystyle \sA$ & A set\\
$\displaystyle \R$ & The set of real numbers \\
$\displaystyle \{0, 1\}$ & The set containing 0 and 1 \\
$\displaystyle \{0, 1, \dots, n \}$ & The set of all integers between $0$ and $n$\\
$\displaystyle [a, b]$ & The real interval including $a$ and $b$\\
$\displaystyle (a, b]$ & The real interval excluding $a$ but including $b$\\
$\displaystyle \sA \backslash \sB$ & Set subtraction, i.e., the set containing the elements of $\sA$ that are not in $\sB$\\
$\displaystyle \gG$ & A graph\\
$\displaystyle \parents_\gG(\ervx_i)$ & The parents of $\ervx_i$ in $\gG$
\end{tabular}
\vspace{0.25cm}


\centerline{\bf Indexing}
\bgroup
\def\arraystretch{1.5}

\begin{tabular}{p{1.25in}p{3.25in}}
$\displaystyle \eva_i$ & Element $i$ of vector $\va$, with indexing starting at 1 \\
$\displaystyle \eva_{-i}$ & All elements of vector $\va$ except for element $i$ \\
$\displaystyle \emA_{i,j}$ & Element $i, j$ of matrix $\mA$ \\
$\displaystyle \mA_{i, :}$ & Row $i$ of matrix $\mA$ \\
$\displaystyle \mA_{:, i}$ & Column $i$ of matrix $\mA$ \\
$\displaystyle \etA_{i, j, k}$ & Element $(i, j, k)$ of a 3-D tensor $\tA$\\
$\displaystyle \tA_{:, :, i}$ & 2-D slice of a 3-D tensor\\
$\displaystyle \erva_i$ & Element $i$ of the random vector $\rva$ \\
\end{tabular}
\egroup
\vspace{0.25cm}


\centerline{\bf Calculus}
\bgroup
\def\arraystretch{1.5}
\begin{tabular}{p{1.25in}p{3.25in}}
% NOTE: the [2ex] on the next line adds extra height to that row of the table.
% Without that command, the fraction on the first line is too tall and collides
% with the fraction on the second line.
$\displaystyle\frac{d y} {d x}$ & Derivative of $y$ with respect to $x$\\ [2ex]
$\displaystyle \frac{\partial y} {\partial x} $ & Partial derivative of $y$ with respect to $x$ \\
$\displaystyle \nabla_\vx y $ & Gradient of $y$ with respect to $\vx$ \\
$\displaystyle \nabla_\mX y $ & Matrix derivatives of $y$ with respect to $\mX$ \\
$\displaystyle \nabla_\tX y $ & Tensor containing derivatives of $y$ with respect to $\tX$ \\
$\displaystyle \frac{\partial f}{\partial \vx} $ & Jacobian matrix $\mJ \in \R^{m\times n}$ of $f: \R^n \rightarrow \R^m$\\
$\displaystyle \nabla_\vx^2 f(\vx)\text{ or }\mH( f)(\vx)$ & The Hessian matrix of $f$ at input point $\vx$\\
$\displaystyle \int f(\vx) d\vx $ & Definite integral over the entire domain of $\vx$ \\
$\displaystyle \int_\sS f(\vx) d\vx$ & Definite integral with respect to $\vx$ over the set $\sS$ \\
\end{tabular}
\egroup
\vspace{0.25cm}

\centerline{\bf Probability and Information Theory}
\bgroup
\def\arraystretch{1.5}
\begin{tabular}{p{1.25in}p{3.25in}}
$\displaystyle P(\ra)$ & A probability distribution over a discrete variable\\
$\displaystyle p(\ra)$ & A probability distribution over a continuous variable, or over
a variable whose type has not been specified\\
$\displaystyle \ra \sim P$ & Random variable $\ra$ has distribution $P$\\% so thing on left of \sim should always be a random variable, with name beginning with \r
$\displaystyle  \E_{\rx\sim P} [ f(x) ]\text{ or } \E f(x)$ & Expectation of $f(x)$ with respect to $P(\rx)$ \\
$\displaystyle \Var(f(x)) $ &  Variance of $f(x)$ under $P(\rx)$ \\
$\displaystyle \Cov(f(x),g(x)) $ & Covariance of $f(x)$ and $g(x)$ under $P(\rx)$\\
$\displaystyle H(\rx) $ & Shannon entropy of the random variable $\rx$\\
$\displaystyle \KL ( P \Vert Q ) $ & Kullback-Leibler divergence of P and Q \\
$\displaystyle \mathcal{N} ( \vx ; \vmu , \mSigma)$ & Gaussian distribution %
over $\vx$ with mean $\vmu$ and covariance $\mSigma$ \\
\end{tabular}
\egroup
\vspace{0.25cm}

\centerline{\bf Functions}
\bgroup
\def\arraystretch{1.5}
\begin{tabular}{p{1.25in}p{3.25in}}
$\displaystyle f: \sA \rightarrow \sB$ & The function $f$ with domain $\sA$ and range $\sB$\\
$\displaystyle f \circ g $ & Composition of the functions $f$ and $g$ \\
  $\displaystyle f(\vx ; \vtheta) $ & A function of $\vx$ parametrized by $\vtheta$.
  (Sometimes we write $f(\vx)$ and omit the argument $\vtheta$ to lighten notation) \\
$\displaystyle \log x$ & Natural logarithm of $x$ \\
$\displaystyle \sigma(x)$ & Logistic sigmoid, $\displaystyle \frac{1} {1 + \exp(-x)}$ \\
$\displaystyle \zeta(x)$ & Softplus, $\log(1 + \exp(x))$ \\
$\displaystyle || \vx ||_p $ & $\normlp$ norm of $\vx$ \\
$\displaystyle || \vx || $ & $\normltwo$ norm of $\vx$ \\
$\displaystyle x^+$ & Positive part of $x$, i.e., $\max(0,x)$\\
$\displaystyle \1_\mathrm{condition}$ & is 1 if the condition is true, 0 otherwise\\
\end{tabular}
\egroup
\vspace{0.25cm}


==> backup/intro.tex <==
One example questions are shown in Figure~\ref{fig:intro-example1}, where the model is asked to solve the question \textit{Study this flowchart of the English, Spanish, and Scottish royal families to identify which two monarchs were related by both blood and marriage.}. 
%The question is accompanied with the options \textit{Phillip II and Mary I, Francis II and Mary Queen of Scots, Elizabeth I and Edward VI, Catherine of Aragon and Henry II}. 
To solve the question, the model needs to take two steps by first collect the required information from the flowchart and then reason about the blood and marriage relations.
% Another example can be found in Figure~\ref{fig:intro-example2}, where the model is asked to solve the question \textit{What is the sum of making progress ,losing ground and same in the year 2011}. This question also involves a two-hop reasoning process, where the first step is to extract the numbers for \textit{making progress}, \textit{losing ground} and \textit{same in the year 2021}. The extracted numbers are summed up in the second step to get the final answer.


This empirical observation therefore, inspires the development of a pipeline that queries VLMs twice with different prompts focused on the data. The first prompt, \textit{Query 1: Please collect the information useful for answering the question}, gathers the necessary details, while the second prompt, \textit{Query 2: Please infer the results with chain-of-thought reasoning using the collected information and image <query 1 input> < query 1 output>}, focuses on drawing conclusions~\cite{DBLP:conf/emnlp/PerezLYCK20} (The place holders \textit{<query 1 input>} and \textit{<query 1 output>} will be filled by the corresponding data during the inference.). The two-step pipeline allows VLMs to utilize the visual perception of vision encoder in the first step and conduct multi-hop reasoning in the second query (an increase of 5.0\% accuracy score in DocVQA dataset)~\cite{DBLP:conf/nips/0001GSC023}. 

We conduct a preliminary experiment, indicating that the state-of-the-art VLMs struggle to accurately answer such questions. In contrast, the underlying LLM component can produce the correct answer when the relevant information is presented in textual form, indicating that the multi-hop reasoning capabilities are diminished when integrating LLMs into VLMs. Following this notion, we attempted to query VLMs multiple times, with the first query aimed at gathering the relevant information from the image and subsequent queries focused on inferring from the collected results. The results suggest that this additional querying approach yields surprising improvements and can help VLMs to have a stronger multi-hop reasoning capability.



The ability to parse logical content is crucial for developing expert AI agents, and this challenge has increasingly attracted researchers' attention in recent years~\cite{yue2024mmmu}. Examples of such content include documents~\cite{DBLP:conf/wacv/MathewKJ21}, infographics~\cite{DBLP:conf/wacv/MathewBTKVJ22}, charts~\cite{DBLP:conf/acl/MasryLTJH22}, and diagrams~\cite{yue2024mmmu}. These types of content often present information in a structured, non-linear fashion, requiring models to combine spatial/visual recognition with multi-hop reasoning to arrive at the correct interpretation or answer.

We borrow the idea of \textit{System 2}, which refers to a complex inference process in LLMs. The \textit{System 2} can be distilled into \textit{System 1}, which uses a streamlined and efficient inference process~\cite{yu2024distilling}. We implement our \textit{System 1} as a vanilla inference pipeline that queries the VLM only once~\cite{yu2024distilling}. To distill \textit{System 1}, we generate and store the oracle representation of \textit{System 2} using the two-query pipeline. Since both systems use the identical model, we can directly use the \textit{System 2} representation to supervise the learning of \textit{System 1}. As a result, the distilled \textit{System 1} can learn the rich inference patterns encoded in the representation space and perform efficient inference.


==> math_commands.tex <==
%%%%% NEW MATH DEFINITIONS %%%%%

\usepackage{amsmath,amsfonts,bm}

% Mark sections of captions for referring to divisions of figures
\newcommand{\figleft}{{\em (Left)}}
\newcommand{\figcenter}{{\em (Center)}}
\newcommand{\figright}{{\em (Right)}}
\newcommand{\figtop}{{\em (Top)}}
\newcommand{\figbottom}{{\em (Bottom)}}
\newcommand{\captiona}{{\em (a)}}
\newcommand{\captionb}{{\em (b)}}
\newcommand{\captionc}{{\em (c)}}
\newcommand{\captiond}{{\em (d)}}

% Highlight a newly defined term
\newcommand{\newterm}[1]{{\bf #1}}


% Figure reference, lower-case.
\def\figref#1{figure~\ref{#1}}
% Figure reference, capital. For start of sentence
\def\Figref#1{Figure~\ref{#1}}
\def\twofigref#1#2{figures \ref{#1} and \ref{#2}}
\def\quadfigref#1#2#3#4{figures \ref{#1}, \ref{#2}, \ref{#3} and \ref{#4}}
% Section reference, lower-case.
\def\secref#1{section~\ref{#1}}
% Section reference, capital.
\def\Secref#1{Section~\ref{#1}}
% Reference to two sections.
\def\twosecrefs#1#2{sections \ref{#1} and \ref{#2}}
% Reference to three sections.
\def\secrefs#1#2#3{sections \ref{#1}, \ref{#2} and \ref{#3}}
% Reference to an equation, lower-case.
\def\eqref#1{equation~\ref{#1}}
% Reference to an equation, upper case
\def\Eqref#1{Equation~\ref{#1}}
% A raw reference to an equation---avoid using if possible
\def\plaineqref#1{\ref{#1}}
% Reference to a chapter, lower-case.
\def\chapref#1{chapter~\ref{#1}}
% Reference to an equation, upper case.
\def\Chapref#1{Chapter~\ref{#1}}
% Reference to a range of chapters
\def\rangechapref#1#2{chapters\ref{#1}--\ref{#2}}
% Reference to an algorithm, lower-case.
\def\algref#1{algorithm~\ref{#1}}
% Reference to an algorithm, upper case.
\def\Algref#1{Algorithm~\ref{#1}}
\def\twoalgref#1#2{algorithms \ref{#1} and \ref{#2}}
\def\Twoalgref#1#2{Algorithms \ref{#1} and \ref{#2}}
% Reference to a part, lower case
\def\partref#1{part~\ref{#1}}
% Reference to a part, upper case
\def\Partref#1{Part~\ref{#1}}
\def\twopartref#1#2{parts \ref{#1} and \ref{#2}}

\def\ceil#1{\lceil #1 \rceil}
\def\floor#1{\lfloor #1 \rfloor}
\def\1{\bm{1}}
\newcommand{\train}{\mathcal{D}}
\newcommand{\valid}{\mathcal{D_{\mathrm{valid}}}}
\newcommand{\test}{\mathcal{D_{\mathrm{test}}}}

\def\eps{{\epsilon}}


% Random variables
\def\reta{{\textnormal{$\eta$}}}
\def\ra{{\textnormal{a}}}
\def\rb{{\textnormal{b}}}
\def\rc{{\textnormal{c}}}
\def\rd{{\textnormal{d}}}
\def\re{{\textnormal{e}}}
\def\rf{{\textnormal{f}}}
\def\rg{{\textnormal{g}}}
\def\rh{{\textnormal{h}}}
\def\ri{{\textnormal{i}}}
\def\rj{{\textnormal{j}}}
\def\rk{{\textnormal{k}}}
\def\rl{{\textnormal{l}}}
% rm is already a command, just don't name any random variables m
\def\rn{{\textnormal{n}}}
\def\ro{{\textnormal{o}}}
\def\rp{{\textnormal{p}}}
\def\rq{{\textnormal{q}}}
\def\rr{{\textnormal{r}}}
\def\rs{{\textnormal{s}}}
\def\rt{{\textnormal{t}}}
\def\ru{{\textnormal{u}}}
\def\rv{{\textnormal{v}}}
\def\rw{{\textnormal{w}}}
\def\rx{{\textnormal{x}}}
\def\ry{{\textnormal{y}}}
\def\rz{{\textnormal{z}}}

% Random vectors
\def\rvepsilon{{\mathbf{\epsilon}}}
\def\rvtheta{{\mathbf{\theta}}}
\def\rva{{\mathbf{a}}}
\def\rvb{{\mathbf{b}}}
\def\rvc{{\mathbf{c}}}
\def\rvd{{\mathbf{d}}}
\def\rve{{\mathbf{e}}}
\def\rvf{{\mathbf{f}}}
\def\rvg{{\mathbf{g}}}
\def\rvh{{\mathbf{h}}}
\def\rvu{{\mathbf{i}}}
\def\rvj{{\mathbf{j}}}
\def\rvk{{\mathbf{k}}}
\def\rvl{{\mathbf{l}}}
\def\rvm{{\mathbf{m}}}
\def\rvn{{\mathbf{n}}}
\def\rvo{{\mathbf{o}}}
\def\rvp{{\mathbf{p}}}
\def\rvq{{\mathbf{q}}}
\def\rvr{{\mathbf{r}}}
\def\rvs{{\mathbf{s}}}
\def\rvt{{\mathbf{t}}}
\def\rvu{{\mathbf{u}}}
\def\rvv{{\mathbf{v}}}
\def\rvw{{\mathbf{w}}}
\def\rvx{{\mathbf{x}}}
\def\rvy{{\mathbf{y}}}
\def\rvz{{\mathbf{z}}}

% Elements of random vectors
\def\erva{{\textnormal{a}}}
\def\ervb{{\textnormal{b}}}
\def\ervc{{\textnormal{c}}}
\def\ervd{{\textnormal{d}}}
\def\erve{{\textnormal{e}}}
\def\ervf{{\textnormal{f}}}
\def\ervg{{\textnormal{g}}}
\def\ervh{{\textnormal{h}}}
\def\ervi{{\textnormal{i}}}
\def\ervj{{\textnormal{j}}}
\def\ervk{{\textnormal{k}}}
\def\ervl{{\textnormal{l}}}
\def\ervm{{\textnormal{m}}}
\def\ervn{{\textnormal{n}}}
\def\ervo{{\textnormal{o}}}
\def\ervp{{\textnormal{p}}}
\def\ervq{{\textnormal{q}}}
\def\ervr{{\textnormal{r}}}
\def\ervs{{\textnormal{s}}}
\def\ervt{{\textnormal{t}}}
\def\ervu{{\textnormal{u}}}
\def\ervv{{\textnormal{v}}}
\def\ervw{{\textnormal{w}}}
\def\ervx{{\textnormal{x}}}
\def\ervy{{\textnormal{y}}}
\def\ervz{{\textnormal{z}}}

% Random matrices
\def\rmA{{\mathbf{A}}}
\def\rmB{{\mathbf{B}}}
\def\rmC{{\mathbf{C}}}
\def\rmD{{\mathbf{D}}}
\def\rmE{{\mathbf{E}}}
\def\rmF{{\mathbf{F}}}
\def\rmG{{\mathbf{G}}}
\def\rmH{{\mathbf{H}}}
\def\rmI{{\mathbf{I}}}
\def\rmJ{{\mathbf{J}}}
\def\rmK{{\mathbf{K}}}
\def\rmL{{\mathbf{L}}}
\def\rmM{{\mathbf{M}}}
\def\rmN{{\mathbf{N}}}
\def\rmO{{\mathbf{O}}}
\def\rmP{{\mathbf{P}}}
\def\rmQ{{\mathbf{Q}}}
\def\rmR{{\mathbf{R}}}
\def\rmS{{\mathbf{S}}}
\def\rmT{{\mathbf{T}}}
\def\rmU{{\mathbf{U}}}
\def\rmV{{\mathbf{V}}}
\def\rmW{{\mathbf{W}}}
\def\rmX{{\mathbf{X}}}
\def\rmY{{\mathbf{Y}}}
\def\rmZ{{\mathbf{Z}}}

% Elements of random matrices
\def\ermA{{\textnormal{A}}}
\def\ermB{{\textnormal{B}}}
\def\ermC{{\textnormal{C}}}
\def\ermD{{\textnormal{D}}}
\def\ermE{{\textnormal{E}}}
\def\ermF{{\textnormal{F}}}
\def\ermG{{\textnormal{G}}}
\def\ermH{{\textnormal{H}}}
\def\ermI{{\textnormal{I}}}
\def\ermJ{{\textnormal{J}}}
\def\ermK{{\textnormal{K}}}
\def\ermL{{\textnormal{L}}}
\def\ermM{{\textnormal{M}}}
\def\ermN{{\textnormal{N}}}
\def\ermO{{\textnormal{O}}}
\def\ermP{{\textnormal{P}}}
\def\ermQ{{\textnormal{Q}}}
\def\ermR{{\textnormal{R}}}
\def\ermS{{\textnormal{S}}}
\def\ermT{{\textnormal{T}}}
\def\ermU{{\textnormal{U}}}
\def\ermV{{\textnormal{V}}}
\def\ermW{{\textnormal{W}}}
\def\ermX{{\textnormal{X}}}
\def\ermY{{\textnormal{Y}}}
\def\ermZ{{\textnormal{Z}}}

% Vectors
\def\vzero{{\bm{0}}}
\def\vone{{\bm{1}}}
\def\vmu{{\bm{\mu}}}
\def\vtheta{{\bm{\theta}}}
\def\va{{\bm{a}}}
\def\vb{{\bm{b}}}
\def\vc{{\bm{c}}}
\def\vd{{\bm{d}}}
\def\ve{{\bm{e}}}
\def\vf{{\bm{f}}}
\def\vg{{\bm{g}}}
\def\vh{{\bm{h}}}
\def\vi{{\bm{i}}}
\def\vj{{\bm{j}}}
\def\vk{{\bm{k}}}
\def\vl{{\bm{l}}}
\def\vm{{\bm{m}}}
\def\vn{{\bm{n}}}
\def\vo{{\bm{o}}}
\def\vp{{\bm{p}}}
\def\vq{{\bm{q}}}
\def\vr{{\bm{r}}}
\def\vs{{\bm{s}}}
\def\vt{{\bm{t}}}
\def\vu{{\bm{u}}}
\def\vv{{\bm{v}}}
\def\vw{{\bm{w}}}
\def\vx{{\bm{x}}}
\def\vy{{\bm{y}}}
\def\vz{{\bm{z}}}

% Elements of vectors
\def\evalpha{{\alpha}}
\def\evbeta{{\beta}}
\def\evepsilon{{\epsilon}}
\def\evlambda{{\lambda}}
\def\evomega{{\omega}}
\def\evmu{{\mu}}
\def\evpsi{{\psi}}
\def\evsigma{{\sigma}}
\def\evtheta{{\theta}}
\def\eva{{a}}
\def\evb{{b}}
\def\evc{{c}}
\def\evd{{d}}
\def\eve{{e}}
\def\evf{{f}}
\def\evg{{g}}
\def\evh{{h}}
\def\evi{{i}}
\def\evj{{j}}
\def\evk{{k}}
\def\evl{{l}}
\def\evm{{m}}
\def\evn{{n}}
\def\evo{{o}}
\def\evp{{p}}
\def\evq{{q}}
\def\evr{{r}}
\def\evs{{s}}
\def\evt{{t}}
\def\evu{{u}}
\def\evv{{v}}
\def\evw{{w}}
\def\evx{{x}}
\def\evy{{y}}
\def\evz{{z}}

% Matrix
\def\mA{{\bm{A}}}
\def\mB{{\bm{B}}}
\def\mC{{\bm{C}}}
\def\mD{{\bm{D}}}
\def\mE{{\bm{E}}}
\def\mF{{\bm{F}}}
\def\mG{{\bm{G}}}
\def\mH{{\bm{H}}}
\def\mI{{\bm{I}}}
\def\mJ{{\bm{J}}}
\def\mK{{\bm{K}}}
\def\mL{{\bm{L}}}
\def\mM{{\bm{M}}}
\def\mN{{\bm{N}}}
\def\mO{{\bm{O}}}
\def\mP{{\bm{P}}}
\def\mQ{{\bm{Q}}}
\def\mR{{\bm{R}}}
\def\mS{{\bm{S}}}
\def\mT{{\bm{T}}}
\def\mU{{\bm{U}}}
\def\mV{{\bm{V}}}
\def\mW{{\bm{W}}}
\def\mX{{\bm{X}}}
\def\mY{{\bm{Y}}}
\def\mZ{{\bm{Z}}}
\def\mBeta{{\bm{\beta}}}
\def\mPhi{{\bm{\Phi}}}
\def\mLambda{{\bm{\Lambda}}}
\def\mSigma{{\bm{\Sigma}}}

% Tensor
\DeclareMathAlphabet{\mathsfit}{\encodingdefault}{\sfdefault}{m}{sl}
\SetMathAlphabet{\mathsfit}{bold}{\encodingdefault}{\sfdefault}{bx}{n}
\newcommand{\tens}[1]{\bm{\mathsfit{#1}}}
\def\tA{{\tens{A}}}
\def\tB{{\tens{B}}}
\def\tC{{\tens{C}}}
\def\tD{{\tens{D}}}
\def\tE{{\tens{E}}}
\def\tF{{\tens{F}}}
\def\tG{{\tens{G}}}
\def\tH{{\tens{H}}}
\def\tI{{\tens{I}}}
\def\tJ{{\tens{J}}}
\def\tK{{\tens{K}}}
\def\tL{{\tens{L}}}
\def\tM{{\tens{M}}}
\def\tN{{\tens{N}}}
\def\tO{{\tens{O}}}
\def\tP{{\tens{P}}}
\def\tQ{{\tens{Q}}}
\def\tR{{\tens{R}}}
\def\tS{{\tens{S}}}
\def\tT{{\tens{T}}}
\def\tU{{\tens{U}}}
\def\tV{{\tens{V}}}
\def\tW{{\tens{W}}}
\def\tX{{\tens{X}}}
\def\tY{{\tens{Y}}}
\def\tZ{{\tens{Z}}}


% Graph
\def\gA{{\mathcal{A}}}
\def\gB{{\mathcal{B}}}
\def\gC{{\mathcal{C}}}
\def\gD{{\mathcal{D}}}
\def\gE{{\mathcal{E}}}
\def\gF{{\mathcal{F}}}
\def\gG{{\mathcal{G}}}
\def\gH{{\mathcal{H}}}
\def\gI{{\mathcal{I}}}
\def\gJ{{\mathcal{J}}}
\def\gK{{\mathcal{K}}}
\def\gL{{\mathcal{L}}}
\def\gM{{\mathcal{M}}}
\def\gN{{\mathcal{N}}}
\def\gO{{\mathcal{O}}}
\def\gP{{\mathcal{P}}}
\def\gQ{{\mathcal{Q}}}
\def\gR{{\mathcal{R}}}
\def\gS{{\mathcal{S}}}
\def\gT{{\mathcal{T}}}
\def\gU{{\mathcal{U}}}
\def\gV{{\mathcal{V}}}
\def\gW{{\mathcal{W}}}
\def\gX{{\mathcal{X}}}
\def\gY{{\mathcal{Y}}}
\def\gZ{{\mathcal{Z}}}

% Sets
\def\sA{{\mathbb{A}}}
\def\sB{{\mathbb{B}}}
\def\sC{{\mathbb{C}}}
\def\sD{{\mathbb{D}}}
% Don't use a set called E, because this would be the same as our symbol
% for expectation.
\def\sF{{\mathbb{F}}}
\def\sG{{\mathbb{G}}}
\def\sH{{\mathbb{H}}}
\def\sI{{\mathbb{I}}}
\def\sJ{{\mathbb{J}}}
\def\sK{{\mathbb{K}}}
\def\sL{{\mathbb{L}}}
\def\sM{{\mathbb{M}}}
\def\sN{{\mathbb{N}}}
\def\sO{{\mathbb{O}}}
\def\sP{{\mathbb{P}}}
\def\sQ{{\mathbb{Q}}}
\def\sR{{\mathbb{R}}}
\def\sS{{\mathbb{S}}}
\def\sT{{\mathbb{T}}}
\def\sU{{\mathbb{U}}}
\def\sV{{\mathbb{V}}}
\def\sW{{\mathbb{W}}}
\def\sX{{\mathbb{X}}}
\def\sY{{\mathbb{Y}}}
\def\sZ{{\mathbb{Z}}}

% Entries of a matrix
\def\emLambda{{\Lambda}}
\def\emA{{A}}
\def\emB{{B}}
\def\emC{{C}}
\def\emD{{D}}
\def\emE{{E}}
\def\emF{{F}}
\def\emG{{G}}
\def\emH{{H}}
\def\emI{{I}}
\def\emJ{{J}}
\def\emK{{K}}
\def\emL{{L}}
\def\emM{{M}}
\def\emN{{N}}
\def\emO{{O}}
\def\emP{{P}}
\def\emQ{{Q}}
\def\emR{{R}}
\def\emS{{S}}
\def\emT{{T}}
\def\emU{{U}}
\def\emV{{V}}
\def\emW{{W}}
\def\emX{{X}}
\def\emY{{Y}}
\def\emZ{{Z}}
\def\emSigma{{\Sigma}}

% entries of a tensor
% Same font as tensor, without \bm wrapper
\newcommand{\etens}[1]{\mathsfit{#1}}
\def\etLambda{{\etens{\Lambda}}}
\def\etA{{\etens{A}}}
\def\etB{{\etens{B}}}
\def\etC{{\etens{C}}}
\def\etD{{\etens{D}}}
\def\etE{{\etens{E}}}
\def\etF{{\etens{F}}}
\def\etG{{\etens{G}}}
\def\etH{{\etens{H}}}
\def\etI{{\etens{I}}}
\def\etJ{{\etens{J}}}
\def\etK{{\etens{K}}}
\def\etL{{\etens{L}}}
\def\etM{{\etens{M}}}
\def\etN{{\etens{N}}}
\def\etO{{\etens{O}}}
\def\etP{{\etens{P}}}
\def\etQ{{\etens{Q}}}
\def\etR{{\etens{R}}}
\def\etS{{\etens{S}}}
\def\etT{{\etens{T}}}
\def\etU{{\etens{U}}}
\def\etV{{\etens{V}}}
\def\etW{{\etens{W}}}
\def\etX{{\etens{X}}}
\def\etY{{\etens{Y}}}
\def\etZ{{\etens{Z}}}

% The true underlying data generating distribution
\newcommand{\pdata}{p_{\rm{data}}}
% The empirical distribution defined by the training set
\newcommand{\ptrain}{\hat{p}_{\rm{data}}}
\newcommand{\Ptrain}{\hat{P}_{\rm{data}}}
% The model distribution
\newcommand{\pmodel}{p_{\rm{model}}}
\newcommand{\Pmodel}{P_{\rm{model}}}
\newcommand{\ptildemodel}{\tilde{p}_{\rm{model}}}
% Stochastic autoencoder distributions
\newcommand{\pencode}{p_{\rm{encoder}}}
\newcommand{\pdecode}{p_{\rm{decoder}}}
\newcommand{\precons}{p_{\rm{reconstruct}}}

\newcommand{\laplace}{\mathrm{Laplace}} % Laplace distribution

\newcommand{\E}{\mathbb{E}}
\newcommand{\Ls}{\mathcal{L}}
\newcommand{\R}{\mathbb{R}}
\newcommand{\emp}{\tilde{p}}
\newcommand{\lr}{\alpha}
\newcommand{\reg}{\lambda}
\newcommand{\rect}{\mathrm{rectifier}}
\newcommand{\softmax}{\mathrm{softmax}}
\newcommand{\sigmoid}{\sigma}
\newcommand{\softplus}{\zeta}
\newcommand{\KL}{D_{\mathrm{KL}}}
\newcommand{\Var}{\mathrm{Var}}
\newcommand{\standarderror}{\mathrm{SE}}
\newcommand{\Cov}{\mathrm{Cov}}
% Wolfram Mathworld says $L^2$ is for function spaces and $\ell^2$ is for vectors
% But then they seem to use $L^2$ for vectors throughout the site, and so does
% wikipedia.
\newcommand{\normlzero}{L^0}
\newcommand{\normlone}{L^1}
\newcommand{\normltwo}{L^2}
\newcommand{\normlp}{L^p}
\newcommand{\normmax}{L^\infty}

\newcommand{\parents}{Pa} % See usage in notation.tex. Chosen to match Daphne's book.

\DeclareMathOperator*{\argmax}{arg\,max}
\DeclareMathOperator*{\argmin}{arg\,min}

\DeclareMathOperator{\sign}{sign}
\DeclareMathOperator{\Tr}{Tr}
\let\ab\allowbreak


==> meta/commands.tex <==
\newcommand{\mycomment}[1]{
    \noindent
    \fcolorbox{black}{blue!20}{
        \begin{minipage}{0.95\linewidth}
            \textit{#1}
        \end{minipage}
    }
}




\newcommand{\revise}[1]{{\color{blue} #1}}
\newcommand{\guande}[1]{{\color{purple} Guande: #1}}

\newcommand{\panpan}[1]{{\color{orange}{PX: #1}}}

% \newcommand{\todo}[1]



\newcommand{\prompttext}[1]{
    \begin{tcolorbox}[colback=gray!20, colframe=gray!80, boxrule=0.5mm, arc=1mm, left=2mm, right=2mm]
        \texttt{#1}
    \end{tcolorbox}
}

==> meta/release_commands.tex <==
\newcommand{\panpan}[1]{}
\newcommand{\mycomment}[1]{
}




\newcommand{\revise}[1]{#1}
\newcommand{\guande}[1]{Guande: #1}

\newcommand{\prompttext}[1]{
    \begin{tcolorbox}[colback=gray!20, colframe=gray!80, boxrule=0.5mm, arc=1mm, left=2mm, right=2mm]
        \texttt{#1}
    \end{tcolorbox}
}

==> preamble.tex <==
%
% --- inline annotations
%
\newcommand{\red}[1]{{\color{red}#1}}
\newcommand{\todo}[1]{{\color{red}#1}}
\newcommand{\TODO}[1]{\textbf{\color{red}[TODO: #1]}}
% --- disable by uncommenting  
% \renewcommand{\TODO}[1]{}
% \renewcommand{\todo}[1]{#1}



==> sections/deprecated_02_framework.tex <==

\begin{figure*}[h!]
    \centering
            \includegraphics[width=\textwidth]{figures/pipeline.png}
    \caption{The overall framework. We first introduce a rational prompt library to generate $N$ in-context questions. These questions are then recursively fed into the model $K$ times to produce reasoning-guided responses. Then, the obtained responses are utilized for self-fine-tuning, enabling the model to better internalize the reasoning process. To enhance the model’s ability to capture reasoning effectively, we design and add several innovative components into the model architecture, including an intervention adapter for efficient parameter updates, a cross-modal skip connection to facilitate information exchange across different modalities, and an ensemble learning algorithm to synthesize reasoning derived from multiple in-context questions.
    }
    
    % The framework starts with the dual-query paradigm, where two consecutive instruction prompts are used to generate an oracle answer and the corresponding hidden state $h_2$. We have a single-pass inference process, where the intervention module runs parallel and operates on the hidden representation $\hat{h_1}$. The intervention module can be tuned by the mean square error (MSE) and Kullback-Leibler (KL) divergence losses based on the difference between $h_2$ and $\hat{h_1}$. For clarity, we omit the image input to the first query and single-pass inference.}
    % We first decompose the query into two parts: the first information-seeking query and the actual answer-seeking query. The predicted hidden representation $h_2$ before the \textit{Output} layer is collected to tune the intervention module, which directly operates on the hidden $\hat{h_1}$ representation under the single-pass manner.  The intervention module can be tuned by the mean square error (MSE) and Kullback-Leibler (KL) divergence losses.}
    
    %Next, we prompt the multi-modal LLM with an information-seeking query to collect detailed knowledge ($h_1$) that can assist in generating the answers. Then, with the help of $h_1$, we prompt the multi-modal LLM again using the answer-seeking query to obtain the final answer. Later, the model is trained self-supervised by minimizing the loss over learned representation between two prompting stages.  
    % The input text and the image are fed into the multi-modal LLM for the first query. The first query generates the representation $h_1$ in the LLM decoder layers. Then the first response is then fed into the the multi-modal LLM with the prompt and first query's input. The second query generates the representation $h_o$. We tune the multi-modal LLM by using MSE loss over $h_o$ and $h_t$.
    
    \label{fig:framework}
\end{figure*}



\section{Methodology}
\label{sec:framework}
% In this section, we present our self-distillation framework using the ensembled dual-query prompts. This framework distills ensemble dual-query-prompted multi-modal LLMs into a single multi-modal LLM with single-query execution through representation intervention modules. We first describe the dual-query method and prompt design. Then, we detail the self-distillation process and training objectives, followed by the ensemble learning process and its integration. Finally, we present the intervention module designs.

% In this section, we first describe the dual-query paradigm, then proceed to describe the formulation of our self-distillation framework, which is then followed by introducing prompt ensemble learning and a detailed description of the representation intervention module.\looseness=-1
The overview of our proposed self-distillation framework is illustrated in Figure 2. The framework comprises two primary components: the reasoning trace generation pipeline and the self-distillation model architecture. Within the self-distillation model, we incorporate representation intervention modules designed to perform targeted edits directly within a learnable subspace, while keeping the larger model components frozen to maintain computational efficiency. Additionally, a cross-modal skip connection layer is employed to leverage low-level visual features, enhancing the perceptual capabilities of multimodal LLMs. Furthermore, we introduce a diverse reasoning ensemble mechanism, allowing the model to distill knowledge from multiple reasoning pathways generated through distinct prompts. Each prompt emphasizes a unique reasoning perspective during training, collectively boosting the robustness and accuracy of the final predictions. We detail these components further in the subsequent sections.\looseness=-1

% \subsection{Dual-Query Prompting Paradigm}
\subsection{Reasoning Trace Generation Pipeline}
Our self-distillation framework employs a two-step reasoning trace generation pipeline designed specifically for addressing complex visual question answering (VQA) tasks, as illustrated in Figure 2. The primary objective of this pipeline is to systematically decompose complicated reasoning tasks into manageable sub-tasks, thus enhancing the model’s ability to reason comprehensively.

In the first stage, the multi-modal LLM is prompted to parse and extract relevant visual and contextual information from the provided image. Given the complexity of real-world images, explicit visual cues may not always be sufficient. To account for this, we further introduce an inverse information parsing prompt to explicitly encourage the model to identify subtle or implicitly relevant details that may not be immediately visually salient but are nonetheless crucial for comprehensive understanding and reasoning.

In the second stage, the model utilizes the extracted and parsed information from the initial stage to construct detailed chain-of-thought explanations, subsequently deriving the final answer. By clearly separating the phases of information extraction and reasoning, our two-step prompting approach enables the model to effectively manage multi-step reasoning tasks and integrate diverse visual and contextual elements from the image. This structured approach not only fosters deeper reasoning capabilities but also promotes greater interpretability of the model’s reasoning processes.

% The framework starts with a dual-query prompting paradigm, where we query the multi-modal LLM twice to reach the final answer. 
% Specifically, to address complex multi-hop VQA problems (Figure~\ref{fig:exp-example1}), the model first needs to parse the information within the image. Therefore in the first prompt, we ask the model to extract important information from the image. Since some subtle yet not visually salient information may also be useful for the given task, we apply an inverse information parsing prompt to encourage the model to ``think" about what kinds of information might be useful for answering the question. The second prompt utilizes the information parsed in the previous steps to instruct the model to write a chain-of-thought explanation and come up with the final answer.  This dual-query paradigm allows for a comprehensive analysis of the image, combining explicit visual information with inferred contextual details. By separating the information extraction and reasoning processes, our method can handle complex questions that require multi-step reasoning and integration of various image elements. (All the prompts will be included in the appendix). \looseness=-1

% The result of this second step can be directly used as the prediction. \panpan{it would be helpful to provide some illustration here, since this is critical for the reader to understand the necessity of multi-step prompting} \guande{added in intro}

% Thus, $p_1$ prompts the model to parse the image from both textual and visual perspectives.
% The parsed information is then concatenated with the inputs and fed back into the model. We implement 

% The first query is used to generate the intermediate explanations and thought process, which are then used as part of the input to the second query to generate the final answer. For example, in Figure~\ref{fig:method-overview}, when asking the question \textit{What is the page number of the title 'Enrollment' in CONTENTS}, the first query can be asked to parse and answer the question by determining which area in the image should be focused on and what kinds of the information should be extracted. The answer of \textit{locating the contents on the left of the image} is then used for guiding the model to read the left part of the image and generate the final answer as \textit{5}. \panpan{wondering if we can have a better example here, this seems a bit too abstract for me/readers to understand}
% \guande{change the example in figure 1. but it still looks a bit weird. i will search for some better examples}
Formally, we represent the instruction prompts for the two queries as $p_1$ and $p_2$. In the first query, the instruction prompt $p_1$ is concatenated with the input $x$, which consists of both the image and question input. We only focus on the generative multi-modal LLM, which consists of a series of LLM decoder layers and an output layer (referred as $Output$) that transforms the hidden states output by the decoder layer to the probability of the next token. For simplicity, we only consider the last layer and refer to the representation as $h_1$ for the first query (though we use the intermediate layers too). We represent the next token sequence as $y_1$ and the decoded optimal answer as $\hat{y_1}$. Therefore, we have, \looseness=-1
\begin{align}
P(y_1|[p_1 , x]) = Output(h_1) = Output(f([p_1,x])), \\ \hat{y_1} = Decode(P(y_1|[p_1 , x])),
\end{align}
% Since we focus on the generative multi-modal LLM, we can represent the process of the first query below, 
% \panpan{denotation here needs update, for example, what does Output do exactly?} \guande{added}

% where $p_1 $ is the prompt text for the first query, $h_1$ refers to the hidden state, $y_1^*$ refers to the decoded response of the first query, and \textit{Output} refers to the output layer, which converts the hidden states to the probability for the next token. Typically, \textit{Output} includes the decoding layers of the LLM backbone.
% We use the bracket symbol $[p_1, x]$ to represent the concatenation of the input data, e.g., the prompt and actual input. 
% \panpan{this is a common representation and we do not need the bracket to indicate that y is conditioned on delta and x, also can we use symbol other than delta to represent the prompt? what is commonly used in visual prompting papers}
% \guande{I changed to use lowercase p instead}
Then in the second query, we concatenate the first-query answer $\hat{y_1}$, the input $x$ and the prompt $p_2$:  \looseness=-1
\begin{align}
    P(y_2 | [p_1,x, \hat{y_1}, p_2]) = Output(h_2) \\ =  Output(f([p_1,x,\hat{y_1}, p_2])), 2])), \nonumber \\
    \hat{y_2} = Decode(P(y_2 | [p_1,x,\hat{y_1}, p_2]))
    \label{eq:query2}
\end{align}
where $\hat{y_2}$ is the decoded answer and $h_2$ is the hidden state for the second query (We view this representation as an oracle representation for the model to learn from). 
Finally, the hidden states obtained through this pipeline—which encode rich contextual and semantic information, including reasoning knowledge—serve as the ground truth signals used to train our self-distillation model by computing loss functions. 

%We hypothesize that compared with the single KL-Divergence loss, it is easier for the self-distilled model to learn from the representation space. 

% \panpan{i think we need to provide some intuitive explanation about why it might be useful for the model to directly learn the second hidden state} \guande{added} 

% \subsubsection{Visual Prompt Design}

% % To implement our framework, we designed appropriate visual prompts for $p_1$ and $p_2$. 
% We designed a pool of prompts following the dual-query paradigm in our self-distillation framework. The pool of prompts is important for the ensemble learning described in Sec.~\ref{sec:ensemble}.
% To address complex multi-hop VQA problems (Figure~\ref{fig:exp-example1}), we first need to parse the information within the image. Therefore, in the first prompt $p_1$, we ask the model to extract important information from the image. However, some subtle yet not explicitly visible information may also be useful, especially when the image contains excessive information. To address this, we add an inverse information parsing prompt, encouraging the model to ``think" about what kinds of information might be useful for answering the text question. Thus, $p_1$ prompts the model to parse the image from both textual and visual perspectives.
% The parsed information is then concatenated with the inputs and fed back into the model. We implement the second prompt $p_2$ by instructing the multi-modal LLM to write a chain-of-thought explanation, combining the information parsed in the previous steps. The result of this second step can be directly used as the prediction. \panpan{it would be helpful to provide some illustration here, since this is critical for the reader to understand the necessity of multi-step prompting} \guande{added in intro}
% This dual-query paradigm allows for a more comprehensive analysis of the image, combining explicit visual information with inferred contextual details. By separating the information extraction and reasoning processes, our method can handle complex questions that require multi-step reasoning and integration of various image elements. We include all the prompts in the appendix.


\subsection{Self-Distillation Model Architecture}
Following our two-step reasoning trace generation pipeline, we utilize the generated hidden states to enable single-step inference through self-distillation. In our setting, our pipeline produces hidden states $h_1$ from the first reasoning step and $h_2$ from the second step, along with the final answer.
The hidden state $h_2$ contains the reasoning trace information developed through the two-step process. We distill this information into an intervention module $I$ that efficiently captures these reasoning patterns. The module performs a transformation on the hidden state $h$, producing $\hat{h} = h + I(h)$, which approximates $h_2$. This approach allows the model to benefit from the enriched reasoning without requiring the additional computational cost of the second prompting step.


% To reduce computational cost during inference, we propose a distillation method that requires only a single inference step.
Rather than training transformer weights directly, our intervention module operates in parallel to the transformer layer, modifying the hidden representation with minimal architectural changes. In the following subsections, we detail the implementation of the intervention adapter module $I$, describe the vision-language skip connection between the vision encoder and intervention module, and present the loss function for training the intervention adapter $I$.

% \subsection{Self-Distillation Model Architecture}
% Shown in Figure~\ref{fig:framework}, our reasoning trace generation pipeline generates the answer and the hidden states $h_1$ and $h_2$ for generating the answer. The proceduced final hidden state $h_2$ that leads to the answer in VQA problems.
% To fully use the knwoledge in the hidden state $h_2$, we propose a distillation method based on $h_2$. In the inference step, we only run the model once and we can denote the hidden state as $\hat{h}.$
% Our goal is to bring $\hat{h_1}$ closer to $h_2$, enabling the model to produce the final answer through one-step prompting.
% Since directly training the transformer weights is difficult, we instead apply an intervention on the hidden state. This intervention module takes the hidden state as input and generates a modification, resulting in $\hat{h_1} = h_1 + I(h_1)$, where $\hat{h_1}$ represents the hidden state after incorporating the learned intervention. Essentially, this approach enables the model to perform a "short-cut" in the multi-hop reasoning process, eliminating the need for multiple prompting steps by learning to emulate the two-step representation within a single step. 
% In the following subsections, we first detail our implementation of the intervention adapter module $I$. We then describe how we enhance the model's perceptual capabilities by adding a vision-language skip connection between the vision encoder and the intervention module. Finally, we will present the loss function for training the intervention adapter module $I$.

% we aim to distill this knowledge into a conventional single-step inference process. 

% Since our two-step paradigm gives the final hidden state $h_2$ leading to the answer to the VQA problem, we can distill this state into the conventional single-step inference. Essentially, this enables the model to perform a ``short-cut" in the multi-hop reasoning process, thus eliminating the need to perform multiple prompting steps by learning the representation from itself. 

% Following the denotation from the previous section, we denote the first query prompt as $p_1$ and the hidden state for the first query as $h_1$. Our goal is to bring $h_1$ closer to $h_2$, such that it can produce the final answer via one-step prompting. We denote the hidden state after incorporating the learned intervention module as $\hat{h_1}$. Since training the transformer weights is difficult, we can apply an intervention on the hidden state instead of changing the output of the state. The intervention state takes input of the hidden state and generates a modifictaion as $\hat{h_1} = h_1 + I (h_1)$.


\subsubsection{Intervention Adapter $I$}
To implement the intervention adapter $I$ in the self-distillation (Eq.~\ref{eq:loss_intv}), we employ the idea of representation fine-tuning (ReFT) and make it run parallel to the transformer layer. ReFT uses low-rank decomposition to approximate weight updates through smaller parameter matrices, which are inserted as parallel adaptation layers (in transformer block \#m shown in Figure~\ref{fig:framework}). This approach allows for model inference with no additional computational overhead while significantly reducing the number of parameters required for fine-tuning. We adopt this low-rank adaptation by implementing the intervention block as $I_{LoRA} = BA h_1$, where $B \in \mathcal{R}^{r \times k}$ and $A \in \mathcal{R}^{k \times r}$, with $k$ representing the dimension of the hidden states and $r$ being the low rank, which is substantially smaller than $k$. In line with~\cite{DBLP:conf/iclr/HuSWALWWC22}, we initialize $A$ with a random Gaussian distribution and set $B$ as a zero matrix.


% LoRA implements a parameter-efficient fine-tuning strategy by using a low-rank decomposition for an external adapter block, running in parallel with the original model~\cite{DBLP:conf/iclr/HuSWALWWC22}. This approach allows for model inference with no additional computational overhead while significantly reducing the number of parameters required for fine-tuning~\cite{DBLP:conf/iccv/ZhangRA23}. 
% We adopt this low-rank adaptation by implementing the intervention block as $I_{LoRA} = BA h_1$, where $B \in \mathcal{R}^{r \times k}$ and $A \in \mathcal{R}^{k \times r}$, with $k$ representing the dimension of the hidden states and $r$ being the low rank, which is substantially smaller than $k$. In line with~\cite{DBLP:conf/iclr/HuSWALWWC22}, we initialize $A$ with a random Gaussian distribution and set $B$ as a zero matrix.

We further extend the method by adding control over the positions where intervention occurs in the input sequence. We configure the method to intervene at specific prefix and suffix positions, such as modifying only the first or last $k$ positions (where $k$ is a configurable hyperparameter). This position-based approach is motivated by the observation that certain parts of the input sequence often contain more significant or relevant information for the task. By making these intervening positions configurable hyperparameters, users can implement targeted interventions in the model's processing pipeline. As demonstrated in~\cite{DBLP:journal/corr/abs-2404-03592}, this position-based intervention approach achieves smaller gradients during training while reducing parameter size through the use of low-rank subspaces.


% \subsubsection{Vision-Language Skip Connection}
We observe that the multi-modal LLM may struggle with low-level perceptual tasks such as object counting and object detection, which can serve as intermediate steps in multi-hop VQA tasks~\cite{DBLP:conf/cvpr/YuanWJC21}. To address this and better support the in-context learning with the visual reasoning complexity, we propose a simple skip connection schema that embeds the early layer outputs of the vision encoder into the intervention module. This method leverages low-level vision features to enhance multi-modal LLM's perceptual capabilities. Specifically, the intervention module is implemented as $I_{skip} = R^T (W h_1 + b - Rh_1 + Af)$, where $f$ is the feature extracted from the vision encoder, and $A \in \mathcal{R}^{v \times k}$ is the matrix for projecting the visual features into the subspace.


% \begin{align}
%     P(y_t|[p_t , x]) = Output(h_t) = Output(f([p_t,x])),\\
% y_1^* = argmax(P(y_t|[p_t , x])),
% \end{align}
% where $p_t$ refers to the instruction prompt, $h_t$ refers to the representation and $y_t$ refers to the generated tokens during the inference time.
% Our goal is to mitigate the distance of representation space between the dual-query. For simplicity, we measure the distance by the mean squared error loss (Euclidean distance). 
% The framework can be extended by using other distance measurements such as Wasserstein distance~\cite{DBLP:conf/nips/FrognerZMAP15}.
\subsubsection{Distillation Loss}
To train the intervention module $I$, we can use mean squared error (MSE) loss or the Kullback-Leibler (KL) divergence as the learning objective to compute the difference between $h_2$ and $\hat{h_1}$. Here, we first show the result of the MSE loss
\begin{equation}
    \mathcal{L} = MSE (h_2, \hat{h_1}) 
    \label{eq:loss}
\end{equation}
% To optimize the loss $\mathcal{L}$, we can fine-tune the parameters of the LLM decoder layers. However, the fine-tuning method still requires extensive parameters and may be inefficient for the limited data. Instead, we employ representation fine-tuning (ReFT)~\cite{DBLP:journal/corr/abs-2404-03592} by implementing an adapter module that runs parallel to the transformer layer and adjusts the hidden state.
Since our intervention adapter module $I$ runs parallel with the transformer layers, we can optimize the module only as,
% Our intervention module $I$ modifies the representation as $\hat{h_1} = I(h_1) + h_1$.
Therefore, ~\ref{eq:loss} can be expanded as,
\begin{equation}
    \mathcal{L} = MSE (h_2, I(h_1) + h_1).
    \label{eq:loss_intv}
\end{equation} 
For the KL-divergence, we can include an additional loss term as $\mathcal{L}_{kl} = KL (Output(h_2), Output(I(h_1) + h_1)),$,
%\begin{equation}
%    \mathcal{L} = KL (Output(h_2), %Output(I(h_1) + h_1)),
%\end{equation}
where $Output$ refers to the output layer, which transforms the hidden representation to the token probability. We combine the two losses to improve the performance of the self-distilled model. \looseness=-1
% \panpan{since we include KL-divergence as well , suggest adding it in the formulation}



Therefore, the loss $\mathcal{L}$ can be optimized for the intervention module $I$, which has fewer parameters compared with the decoder layer. The framework is illustrated in Figure~\ref{fig:framework}. 

Equation~\ref{eq:loss_intv} is specific to one layer of fine-tuning. However, we can generalize the framework into multiple layers by adding up the losses for different layers. In our implementation, we only intervene in the last $k$ ($k=3$) layers because the later layers encode the high-level features.
% an intervention module $I$, which mitigate the gap between $P(y_1|[p_1 , x])$ and $P(y_2 | [p_1,x,y_1^*, p_2])$ as $P(y_I| [p_I, x]) = Output(h_1+I(p_I,x))$.
% We train the intervention/mapping by the manually-crafted prompts and the auto-created $y_1^*$, which can be manually validated.

% $P(y_I| [p_I, x]) = Output(h_1+I(p_I,x))$

% Following~\cite{DBLP:journal/corr/abs-2404-03592, DBLP:conf/iclr/HuSWALWWC22}, we implement the intervention adapter $I$ in Eq.~\ref{eq:loss_intv} based on the concept of low-rank decomposition. 
% 


% Since we work on the multi-modal LLM, we further add a bridge between the vision tower and the transformer. Specifically, we connect the hidden states of the vision transformer to the intervention modules, which operates on the hidden states of the transformer layers. Therefore, we can represent the invention as 

% \section{Implementation with Representation Fine-Tuning}
% We extended ReFT ~\cite{DBLP:journal/corr/abs-2404-03592} to implement the intervention module in Eq.~\ref{eq:loss_intv}, and compared it with LoRA fine-tuning~\cite{DBLP:conf/iclr/HuSWALWWC22} as the baseline.
% The construction and flexibility of ReFT allow us to further incorporate a vision-language skip connection as a mixed-module design to further enhance performance. We provide detailed ablation study in the end to evaluate the effectiveness of each method.

% \subsubsection{Background: LoRA and ReFT}


% ReFT is a family of representation intervention methods that directly edits the representation within a subspace. Previous studies have shown that high-level concepts may be encoded and stored in a linear subspace within neural networks~\cite{morris1989parallel}. ReFT directly projects the representation into a linear subspace and edits it directly. We implement ReFT in our framework by $I_{ReFT} = R^T  (W h_1 + b - Rh_1)$, where $R$, $W$ $\in \mathcal{R}^{r\times d}$, where $d$ is the dimension of the low-dimensional subspace. The matrix $R$ needs to be initialized with orthonormal rows to ensure the subspace is linear.


% Furthermore, ReFT aligns more closely with our concept of representation fine-tuning, as it allows for more precise control over which parts of the representation are modified. This targeted approach ensures that the intervention focuses on the most relevant aspects of the model's internal states, leading to potentially more efficient and effective fine-tuning. We illustrate the model structure in Figure~\ref{fig:method-overview}

% \begin{figure}[h]
%     \centering
%     \includegraphics[width=0.5\textwidth]{figures/method-small.pdf}
%     \caption{Self-distillation architecture. The multi-modal LLM takes the sequence containing both text and image tokens. In particular, the text tokens are sent into the LLMs and the image tokens are processed by a vision encoder. Later, we introduce the intervention blocks in LLMs that takes both the learned text embeddings from previous layer and learned visual representations from the vision encoder as input. 
%     % The text tokens and the processed image embeddings are fed into an LLM and the representation of the LLM decoder layer is intervened by the intervention blocks. 
%     We implement a mixed-module design, which uses the simple static intervention in the later layers and ReFT layers in the early layers. }
%     \label{fig:method-overview}
% \end{figure}




\subsection{Diverse Reasoning Ensemble Mechanism}
\label{sec:ensemble}
To enhance the diversity of reasoning traces for improving self-distillation, we employ various prompts to guide vision language models toward reasoning from multiple perspectives. For instance, the prompt ``\textit{To analyze and answer the question, I need to understand the precondition of the question first, then identify what content in the image is relevant to addressing it, working backward from the question to the visual evidence needed}'' targets questions with complex textual reasoning requirements, helping the model parse intricate logical relationships within the text. Conversely, the prompt ``\textit{First, I'll describe the important content in the image, including major objects, people, and text present in the image, then analyze how these visual elements relate to each other and contribute to answering the question}'' addresses visually challenging tasks, particularly those requiring accurate optical character recognition (OCR) and visual detail extraction. These complementary prompting strategies generate diverse reasoning patterns that strengthen the self-distillation process

% \panpan{same as the previous description, we need some intuition or reasoning on why we think ensemble prompt learning will help} \guande{added}


Based on this approach, we first compile a prompt library incorporating with VLM to generate diverse reasoning traces. During training, distinct prompts create varied output hidden state for the same input image and questions, enabling us to train separate representation modules accordingly. After obtaining these trained representation modules, we introduce a weighting module. We implement the weighting modules as a three-layer multi layer perceptron. Specifically, we select the reasoning trace with the highest next-token confidence - determined by top-token probability - as the label to train the weighting module. The underlying assumption here is that higher skewness in token probability distribution indicates greater model confidence [9, 10]. 

During the inference, The process is characterized by the following equation:\looseness=-1
\begin{equation}
    \hat{h_1} = f(x) + \sum_{i\in |A|} w^i I^i (f(x)),
\end{equation}

where $I^i$ denotes the individual intervention module, and $w^i$ refers to the trained wights for each intervention module with the diverse reasoning traces knowledge provided by various prompts.


% Different instruction prompts elicit distinct capabilities and influence LLM behavior differently ~\cite{DBLP:journals/tacl/MizrahiKMDSS24}. For instance, with our two-step prompting pipeline, the first-query prompt ``\textit{analyze which region may be helpful for answering the question}'' guides the multi-modal LLM to identify relevant areas in large documents, while ``\textit{analyze the question to determine what kinds of information may be helpful}'' better supports multi-hop reasoning for simpler images.
% Recent studies show that a single prompt may not be sufficient to solve diverse problems. For example, the prompt elicitating the reasoning process may be useful for the multi-hop reasoning problem, while not suitable for the OCR questions.
% Recent studies have employed the ensemble prompt to achieve more comprehensive model capabilities~\cite{DBLP:conf/aaai/ZhangLWSWWC24, DBLP:journals/corr/abs-2310-00035}.
% Following this idea, we first create a pool of prompts, each consisting of a the first-query prompt and second-query prompt as $\Gamma = \{\{p^1_1, p^1_2\}, \{p^2_1, p^2_2\}, \cdots, \{p^k_1, p^k_2\}\}$. 
% The different pairs of prompts can be used in our two-step prompting pipeline to generate the reasoning traces.
% Following Eq.~\ref{eq:loss_intv}, we can obtain a set of intervention modules $A = {I^1, I^2, \dots, I^k}$ corresponding to the prompts' reasoning traces. 
% % In running the inference, Different interventions modules use the shared same prompt in the inference processs for generating the intervened hidden state $\hat{h_1}$.
% To ensemble these modules during inference, we introduce a weighting module $\sigma$, which produces a set of weights $W = {w^1, w^2, \cdots, w^k} = \sigma(h)$, where $h$ denotes the input representation. The final inference process is then characterized by the following equation:\looseness=-1
% \begin{equation}
%     \hat{h_1} = f(x) + \sum_{i\in |A|} w^i I^i (f(x)),
% \end{equation}
% The weighting module decides \textit{how reliable one intervention module is for the input question.} To train the weighting module $\sigma$, we can use the confidence of the reasoning trace as the oracle label and optimize the corresponding loss. 
% Specifically, we first evaluate the confidence of each reasoning trace using the top token probability values, under the assumption that a higher skewness in probability distribution indicates greater model confidence~\cite{DBLP:conf/icml/GuoPSW17, DBLP:conf/naacl/GengCWKNG24}. For each two-step prompt $i$, we compute its confidence score as $c_i = \max(P_i)$ at the last token position ($P_i$ refers to the next token probability using the prompt $\{p^i_1, p^i_2\}$). Then, we can define the loss as:
% $L_{weight} = |\sigma(h) - \text{softmax}(\mathbf{c})|_2$
% where $\mathbf{c} = [c_1, ..., c_{|A|}]$ are the confidence scores. We implement the weighting module $\sigma$ as a three-layer multi-layer perceptron (MLP) with the same dimension of the hidden layers as the representation of $\hat{h_1}$
% This training procedure ensures that the weighting module learns to assign appropriate weights based on the dual-query prompt's confidence. Furthermore, we also incorporate the MSE loss from Eq.~\ref{eq:loss_intv} when training the weighting module to ensure that the ensemble output maintains accuracy and consistency with the expected results.

% This ensures the weighting module learns to assign higher weights to more confident predictions during inference.
% These confidence values are then used as the ground-truth labels for the weighting module. The input to the weighting module is the representation $h$, and the output is the set of weights $W$ used to ensemble the intervention modules during inference. 

% \panpan{a bit unclear on how the training loss looks like and how the probability values are utilized, do we use the probability of every output tokens ? how is input representation mapped to weights?} \guande{revised}


==> sections/deprecated_03_implementation.tex <==
\section{Implementation with Representation Fine-Tuning}


In this section, we present our implementations for the intervention modules. Building on Equation~\ref{eq:loss_intv}, the intervention module is optimized towards the result generated by the query-twice method. To achieve this, the intervention module $I$ is designed to be minimized, allowing for a reduced number of parameters. We explore two implementations based on Low-Rank Adaption (LoRA)~\cite{DBLP:conf/iclr/HuSWALWWC22} and Representation fine-tuning (ReFT)~\cite{DBLP:journal/corr/abs-2404-03592}. Additionally, to bridge the gap between the vision encoder and the LLM, we also propose a vision-language skip connection and mixed-module design to further enhance performance.

\subsection{Representation Fine-Tuning Methods}

\subsubsection{LoRA Baseline}
LoRA implements a parameter-efficient fine-tuning strategy by using a low-rank decomposition for an external adapter block, running in parallel with the original model~\cite{DBLP:conf/iclr/HuSWALWWC22}. This approach allows for model inference with no additional computational overhead while significantly reducing the number of parameters required for fine-tuning~\cite{DBLP:conf/iccv/ZhangRA23}. We adopt this low-rank adaptation by implementing the intervention block as $I_{LoRA} = BA h_1$, where $B \in \mathcal{R}^{r \times k}$ and $A \in \mathcal{R}^{k \times r}$, with $k$ representing the dimension of the hidden states and $r$ being the low rank, which is substantially smaller than $k$. In line with~\cite{DBLP:conf/iclr/HuSWALWWC22}, we initialize $A$ with a random Gaussian distribution and set $B$ as a zero matrix.

\subsubsection{Static Intervention Baseline}
We also adopt a simple intervention baseline with a static vector agnostic to the input. The intervention can be represented as $I_{static} = U (U^T h_1 + v )$, where $U \in \mathcal{R}^{r \times k}$ is an orthonormal matrix projecting to a $k$-dimensional subspace and $v$ is a static vector within this subspace. This method is similar to representation engineering, which differently uses PCA to project the original representation~\cite{DBLP:journals/corr/abs-2310-01405}. \panpan{i am not sure if we want to include the static intervention baseline, it might trigger more questions  - like how the static vector is generated - than serve the main narrative} \guande{Static vector is generated in the same way by KL+MSE loss. I can remove it or move it to appendix.}


\subsubsection{ReFT}
ReFT is a family of representation intervention methods that directly edits the representation within a subspace. Previous studies have shown that high-level concepts may be encoded and stored in a linear subspace within neural networks~\cite{morris1989parallel}. Following this notion, ReFT directly projects the representation into a linear subspace and edits it directly. We implement ReFT in our framework by $I_{ReFT} = R^T  (W h_1 + b - Rh_1)$, where $R$, $W$ $\in \mathcal{R}^{r\times d}$, where $d$ is the dimension of the low-dimensional subspace. The matrix $R$ needs to be initialized with orthonormal rows to ensure the subspace remains linear.


ReFT further extends the method by adding control on the position of the inputs. Following~\cite{DBLP:journal/corr/abs-2404-03592}, we configure the method by setting the positions defined by the prefix and suffix positions, such as intervening in the first or last $k$ positions ($k$ can be set as the hyper-parameter). This approach is based on the assumption that partial intervention can be useful when specific parts of the input sequence carry more significant or relevant information for the task. The intervening positions are hyperparameters configurable by the users, allowing for targeted intervention in the model's processing.

Compared to LoRA, ReFT can achieve even smaller gradients during the training process by leveraging position-based intervention and reducing parameter size through the use of low-rank subspaces. Furthermore, ReFT aligns more closely with our concept of representation fine-tuning, as it allows for more precise control over which parts of the representation are modified. This targeted approach ensures that the intervention focuses on the most relevant aspects of the model's internal states, leading to potentially more efficient and effective fine-tuning. We illustrate the model structure in Figure~\ref{fig:method-overview}






% We also adopt a simple intervention baseline with the static vector agnostic to the input. The intervention can be represented as $I_{static} = U (U^T h_1 + v )$, $U \in \mathcal{R}^{r \times k}$ is the orthonormal matrix projecting to a $k$-dimension subspace where $v$ is a static vector within the subspace. Such method is similar to the representation engineering which differently uses PCA to project the original representation


\begin{figure}[h]
    \centering
    \includegraphics[width=0.5\textwidth]{figures/model.pdf}
    \caption{Method overview. The VLM takes the sequence containing both text and image tokens. The image token is processed by a vision encoder, where the internal representation is fed into the intervention blocks through the skip connection. The text tokens and the processed image embeddings are fed into an LLM and the representation of the LLM decoder layer is intervened by the intervention blocks. We implement a mixed-module design, which uses the simple static intervention in the later layers and ReFT layers in the early layers. }
    \label{fig:method-overview}
\end{figure}

\subsection{Vision-Language  Skip Connection, and Mixed-Module Designs}
% \subsection{Vision}
While VLMs achieve state-of-the-art performance on high-level VQA datasets, we observe that VLMs may still struggle with low-level perceptual tasks such as object counting and object detection, which can serve as intermediate steps in multi-hop VQA tasks~\cite{DBLP:conf/cvpr/YuanWJC21}. To address this, we propose a simple skip connection schema that embeds the early layer outputs of the vision encoder into the intervention module. This method leverages low-level vision features to enhance VLM's perceptual capabilities. Specifically, the intervention module is implemented as $I_{skip} = R^T (W h_1 + b - Rh_1 + Af)$, where $f$ is the feature extracted from the vision encoder, and $A \in \mathcal{R}^{v \times k}$ is the matrix for projecting the visual features into our subspace.

% Given the redundancy in LLM layers, we propose to further reduce the inference overhead with skip-layer mechanisms~\cite{DBLP:conf/nips/ZhouXGM0W20}. Since our optimization objective in Equation~\ref{eq:final} is based on the last layers, the skip-layer approach can be used to optimize the inference process without compromising the training objective.

Since we can intervene in the different layers simultaneously, we can mix the different interventions among the different layers. LLMs encode the high-level information in the later layers and therefore, the representation in the later layers can be more structured and close to linear. Following this notion, we propose to apply the static intervention on the later layers while using ReFT in the early layers. Therefore, we can exploit the strong intervention capability of ReFT and the interpretability of static vectors simultaneously. We show the mixed-module design and other modules in Figure~\ref{fig:method-overview}



==> tables/ablation_n.tex <==
\begin{table*}[]
\centering

\begin{tabular}{|c|c|c|c|c|}
\hline
Training          & Model & N Samples & DocVQA & Infographic-VQA \\ \hline
Self-Distillation & ReFT  & 100       &  59.9   &       41.2          \\ \hline
Self-Distillation & ReFT  & 200       &    63.1  &     42.0            \\ \hline
Self-Distillation & ReFT  & 400       &    \textbf{63.5}   &    44.2           \\ \hline
Self-Distillation & ReFT  & 800       &     63.3  & \textbf{44.7}          \\ \hline
\end{tabular}
\caption{Ablative study for the number of ensemble members used in fine-tuning process.}
\label{tab:ablation_n}


\end{table*}

==> tables/ablation_tuned.tex <==
\begin{table}[]
\centering
\begin{tabular}{|c|c|c|c|c|}
\hline
Training          & Model    & Oracle Prompt & DocVQA & Infographic-VQA \\ \hline
N/A               & Baseline & N/A           &        &                 \\ \hline
Self-Distillation & ReFT     & Single        &        &                 \\ \hline
Self-Distillation & ReFT     & Multi         &        &                 \\ \hline
Self-Distillation & LoRA     & N/A           &        &                 \\ \hline
\end{tabular}
\caption{Ablation study for the fine-tuned model.}
\label{tab:ablation_tuned}
\end{table}
